Detailed Avatar Recovery from Single Image

This paper presents a novel framework to recover \emph{detailed} avatar from a single image. It is a challenging task due to factors such as variations in human shapes, body poses, texture, and viewpoints. Prior methods typically attempt to recover the human body shape using a parametric-based template that lacks the surface details. As such resulting body shape appears to be without clothing. In this paper, we propose a novel learning-based framework that combines the robustness of the parametric model with the flexibility of free-form 3D deformation. We use the deep neural networks to refine the 3D shape in a Hierarchical Mesh Deformation (HMD) framework, utilizing the constraints from body joints, silhouettes, and per-pixel shading information. Our method can restore detailed human body shapes with complete textures beyond skinned models. Experiments demonstrate that our method has outperformed previous state-of-the-art approaches, achieving better accuracy in terms of both 2D IoU number and 3D metric distance.

==> coverletter.tex <==
Dear Editors and Reviewers,
Enclosed is our submission to the TPAMI and a previous version of this paper has been published in CVPR 2019 as oral presentation. The previous version is also attached.

In this submission, we have extended the human shape recovery by synthesizing complete texture from a single image, which is illustrated in Section 4. To restoring fully textured human body from a single image, we proposed to utilize appearance flow to predict invisible part from the current view, followed by a symmetry aware texture refinement net to hallucinate the missing part. We did both qualitative and quantitative evaluation. As demonstrated in the experiments in Sec 5.7, we are able to generate the complete texture which is visually pleasing.  In the experiment of shape recovery part, we supplement the 3D joint error evaluation on Human 3.6M dataset, and render our model in the side view to show the recovered shape more intuitively.


Thank you for your consideration.

Authors




To Editors and Reviewers, 
We are submitting an extended version of our CVPR 2019 paper on Human Mesh Recovery, which was the first attempt of using a deep learning approach for photometric stereo and won the best workshop paper prize. 
We have fully revised the manuscript and present new additional contents. This version of the paper includes the following extensions: 
	We have re-designed the network architecture for simultaneous estimation of both surface normal and BRDFs, while the previous method was limited to surface normal estimation. 
	We show an application of re-lighting scenes under a novel light condition to demonstrate the effectiveness of our method. The results are assessed both qualitatively and quantitatively. 
	The whole paper is rewritten to reflect above changes and deliver more details. 
This paper would interest people who are familiar with: 
	Photometric 3D modeling 
	Computational photography / imaging / illumination 
	Low- and mid-level vision 

Thank you for your considerations. 

Authors





